Generalization Guarantee of Training Graph Convolutional Networks with Graph Topology Sampling

Graph convolutional networks (GCNs) have recently achieved great empirical success in learning graph-structured data. To address its scalability issue due to the recursive embedding of neighboring features, graph topology sampling has been proposed to reduce the memory and computational cost of training GCNs, and it has achieved comparable test performance to those without topology sampling in many empirical studies. To the best of our knowledge, this paper provides the first theoretical justification of graph topology sampling in training (up to) three-layer GCNs for semi-supervised node classification. We formally characterize some sufficient conditions on graph topology sampling such that GCN training leads to a diminishing generalization error. Moreover, our method tackles the nonconvex interaction of weights across layers, which is under-explored in the existing theoretical analyses of GCNs. This paper characterizes the impact of graph structures and topology sampling on the generalization performance and sample complexity explicitly, and the theoretical findings are also justified through numerical experiments.

==> sampling.tex <==
\section{Training two(three)-layer GCNs with  sampling}\label{sec: sampling}

\PY{The flow is a bit weird. Will all-node sampling reduce to w/o sampling? If so, we can directly mention the results with sampling}

We considered the case that $\bfA^*$ equals to $\bfA$ in the target function in Sections xx and xx. In practice, this might not always hold as $\bfA^*$ represents the correlations among node labels.  On the other hand, 
Graph sampling can reduce the memory and computational cost in training GCNs, where in each SGD iteration, instead of using the whole graph $\mathcal{G}$, a subset of nodes and/or edges are sampled, and the embedding aggregation is based on the sampled graph rather than $\mathcal{G}$. Mathematically, sampling corresponds to setting some entries in $\bfA$ to zero and scaling the rest when computing the gradient. For example, if node $i$ is not sampled, then the $i$th column of $\bfA$ is all set to $0$. %If an edge $(i,j)$ is not sampled, 
Surprisingly, graph sampling does not degrade the generalization performance in some cases. Here we provide one theoretical explanation of these empirical success.  Moreover, we consider the general case that $\bfA^*$ in the target functions \ref{eqn:concept} and \ref{eqn:concept2} is not necessarily the same as $\bfA$. % and the high-level idea is the with a proper sampling strategy, the resulting matrix may be more similar to $\bfA^*$ than $\bfA$, leading to a desired learning and generalization performance. 

%A=A*, sampling to reduce the memory and computation
%In each SGD iteration, pick a subset of nodes,  equivalent to setting the columns of A with respect to the unsamples nodes to 0 and scale the sampled nodes accordingly.

%We consider A*=AP*, shows that the for a proper sampling stratery, with sampling can still train a neural network with epsilon error even if the number of samples nodes in each iteration is much smaller than the total number of nodes. Our result can be viewed as a theoretical justfication of graph sampling trategies. 

\textbf{The model of $\bfA^*$:} To formalize the analysis,    suppose the node  degrees in $\mathcal{G}$ can be divided into $L$ groups with $L \geq 1$, where the degree of nodes in group $i$ are in the order of $d_l$, i.e., between $cd_l$ and $Cd_l$ for some constants $c \leq C$, and $d_l$ is order-wise smaller than $d_{l+1}$, i.e.,  $d_l=o(d_{l+1})$. Let $N_l$ denote the number of nodes in group $l$. Consider a diagonal matrix $\bfP^*$ where a diagonal entry equals to $p_l^*$ if the corresponding node belongs to group $l$. Our results applies to 
all $\bfA^*=\bfA\bfP^*$ where $p^*_l$ satisfies the following for some positive constant $c_1$ %can be any nonnegative value as long as there exists some constant  $c_1$ such that  %the following is satisfied,

\begin{equation} \label{p_iupper}
  0 \leq  p^*_l\leq  \frac{c_1}{L}\frac{\sum_{i=1}^L d_i \bfN_i}{\sqrt{d_Ld_l}\bfN_l}:= \frac{c_l}{L\Phi_l}, \forall l\in [L] %\frac{c_1}{\max_{n\in[L]}\{\Phi(n,i)\}}=\frac{c_1}{\Phi(L,i)}=c_1\sqrt{\frac{d_i^G}{d_L^G}}\frac{\sum_{l=1}^L d_l^G |\bfN_l|}{d_i^G|\bfN_i|}, 
\end{equation}
 
From \ref{p_iupper}, $\Phi_l$  is proportional to $\sqrt{d_l}N_l$. If a graph is highly unbalanced in the sense that there exists some group $\hat{l}$ such that $\sqrt{d_{\hat{l}}} N_{\hat{l}}\gg  \sqrt{d_l}N_l$ for all other $l$, then $p^*_\hat{l}$ needs to be smaller than other $p^*_l$ from   (\ref{p_iupper}). That means $\bfA^*$ is more balanced than $\bfA$.  That is intuitive because sampling on a highly unbalanced graph could 
not maintain the generalization capability if some important nodes are not sampled.
 
 
  We remark that (\ref{p_iupper}) is a minor condition for most graphs.  
  %$\Phi_l$ increases as $l$ increases. Thus, the upper bound on the right-hand side of (\ref{p_iupper})  is smaller for a higher-degree group.
  To see this, suppose $L$ is a constant, and every $N_l$ is in the order of $N$. % suppose $L\Phi_L$ is a constant (does not scale with $N$),
  Then all constant values % or smaller
  satisfy  (\ref{p_iupper}), and our results hold for many $\bfA^*$. A special example is that $p^*_l=1$ for all $l$, i.e., $\bfA^*=\bfA$.   
  
 
%  because if $\bfA^*$ has some entries significantly larger than others, then not sampling these corresponding nodes would lead to significant errors, no matter how large the number of sampled nodes is.  
%Intuitively,  (\ref{p_iupper}) means that our results apply to $\bfA^*$ that have roughly balanced entries. 
%That is reasonable because if $\bfA^*$ has some entries significantly larger than others, then not sampling these corresponding nodes would lead to significant errors, no matter how large the number of sampled nodes is.  Then with a balanced $\bfA^*$, sampling partial nodes may not introduce too much error in generalization as long as the number of sampled nodes is large enough. 

%if $A$ has entries that are significantly larger than others, then $\bfA^*$ tends to have more balanced entries than that in $\bfA$.   

%Consider an example that  $L$ is a constant, and $d_LN_L \gg d_lN_l$ for any $l \neq L$, which means that a dominating number of edges has at least one end incident to  the highest-degree group.    (\ref{p_iupper}) requires $p^*_l$ to be a constant. Then $p^*_l=1$    $\forall l$  satisfies (\ref{p_iupper}).   $\bfA^*$ can be $\bfA$. 

%Suppose that node degrees of the graph can be divided into $L$ different orders with regard to the number of nodes $N$, where $L=\Theta(1)$. Each group is denoted by $\bfN_i$. Hence, $\sum_{i=1}^{L}|\bfN_i|=N$. Denote the number of nodes sampled in each group as $l_i$. We have $\sum_{i=1}^L l_i=N_{\text{layer}}$. Denote the group with the $i$-th smallest degree as $d^G_{i}$, where $i\in[L]$.\\
\textbf{Sampling strategy and the training algorithms:} We implement a group-wise uniform sampling strategy, where $l_l$ out of $N_l$ nodes are sampled uniformly from each group $l$. Let $\bfA^t$ denote the sampled matrix in the $t$th iteration. %Let $\hat{\bfP}^t$ be a diagonal matrix. 
If node $i$ is sampled in this iteration and  belongs to group $l$ for any $i$ and $l$, the $i$th diagonal entry of a  diagonal matrix $\hat{\bfP}^t$ is $\hat{p}_lN_l/l_l$. Otherwise, the corresponding entry is $0$. Then $\bfA^t=\bfA \hat{\bfP}^t$.

The training algorithms for two (three)-layer GCNs with sampling are summarized in Algorithms xx and xx, respectively. The only difference from those without sampling (Algorithms xx and xx) is that in each SGD iteration $t$, $\bfA^t$ rather than $\bfA$ is used in computing the gradient. 

%With probability $\hat{p}_i$, we choose the group $i$. Apply uniform sampling with replacement within the group $i$ to acquire $l_i$ nodes. Denote the set of indices of sampled nodes in the group $i$ as $\bfs_i=\{s_{i_1}, s_{i_2}, \cdots, s_{i_{l_i}}\}$ and thus $|\bfs_i|=l_i$. Let $p_j=\frac{1}{|\bfN_i|}\hat{p}_i$ for any $i\in \bfN_i$.\\
 
 
 %Theorems \ref{thm:two_sampling} and \ref{thm:three_sampling} state the   performance of training two-layer and three-layer GCNs with a proper sampling strategy discussed in   Assumption \ref{ap_sampling}. 
\begin{assumption}\label{ap_sampling}
(Conditions for sampling)\\
%(1) $\bfA^*$ satisfies  (\ref{p_i''upper}), and $|p_l-\hat{p}_l^*|/\hat{p}_l^*\leq \epsilon^{10}$ for all $l\in[L]$,  
%\begin{equation}
%    l_l \geq \frac{N_l}{1+ \frac{c_l \epsilon ^{10}}{p_l L\Phi_l}}.
%\end{equation}
%(2)
$\bfA^*$ satisfies  (\ref{p_iupper}),   $|\hat{p}_l-p_l^*|/p_l^* =O(\text{poly}(\epsilon))$, and %for all $l\in[L]$,
\begin{equation}\label{eqn:ll}
    l_l \geq \ (1+ \frac{c_l \text{poly}(\epsilon)}{Lp_l \Phi_l})^{-1}N_l \quad \quad \forall l\in[L]
\end{equation}

\end{assumption}

 Assumption \ref{ap_sampling} states the required number of samples in each group. To understand the sampling requirement in (\ref{eqn:ll}) better, consider a special case that %$\bfA^*=\bfA$, which means 
$p^*_l=1$, and $N_l$ is order $N$   for all $l$. Then % for a larger $l$,  $\Phi_l$ is larger , then 
$l_l$ is larger with a larger $d_l$. That means the higher-degree groups are sampled more often than lower-degree groups in this case.  This shares the same intuition as FastGCN \citep{CMX18}, which also samples high-degree nodes with a higher probability. Moreover, the number of sampled nodes $l_l$ can be much smaller than $N_l$, provided  that $p_l$ is small enough. 
%Note that from Assumption \ref{ap_sampling}, the total number of sampled nodes can be much less $N$, as long as $p_l$'s are small, % while the generalization performance is maintained, 
%indicating the success of sampling. 



Theorems \ref{thm:two_sampling} and \ref{thm:three_sampling} state the   generalization guarantees of training two-layer and three-layer GCNs with graph sampling as long as the sampling strategy satisfies % with a proper sampling strategy discussed in
Assumption \ref{ap_sampling}. 
\begin{theorem}(Generalization of training two-layer GCNs with sampling)\label{thm:two_sampling}
 
 If Assumption \ref{ap_sampling} is met, and $\epsilon$, $m$, $n_0$, $\eta$ and $T$ satisfy the requirements in Theorem 
 \label{thm:two}, then 
 
 \begin{equation}%\label{eqn:twolayer}
\mathbb{E}[\frac{1}{T}\sum_{t=1}^{T}\mathbb{E}_{(\bfe_g,\bfX,y)\sim\mathcal{D}}L( F(\bfe_g, \bfX, \bfW^t),y)]\leq    \mathrm{OPT}+\epsilon 
\end{equation}
 \end{theorem}
 where  $\bfW^t$ is the weight matrix returned at iteration $t$. 
 \iffalse
If Assumption \ref{ap_sampling} is met, for every $\epsilon\in(0,K^{-\frac{13}{2}}p^{-4}\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^{-4}(\|\bfA^*\|_\infty+1)^{-4}\|\bfA^*\|_\infty^{-1})$, there exists
\begin{equation}
M_0=\Theta\big(\epsilon^{-6}K^{12}p^{8}\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^{8}(\|\bfA^*\|_\infty+1)^{8}(\|\bfA^*\|_\infty^2+\epsilon^{10})^2\big)
\end{equation}
\begin{equation}
N_0= &\epsilon^{-2} K^7 p^4\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^4(\|\bfA^*\|_\infty^2+1)^2\|\bfA^*\|_\infty^4(1+\delta^2)\log N
\end{equation}
such that  as long as $m\geq M_0$ and $n_0\geq N_0$, choosing $\epsilon_c=\Theta(1)$, $\eta=\Theta(\frac{\epsilon}{m\epsilon_c^2 K(\|\bfA\|_\infty^2+\epsilon^{10}])})$ and $T=\Theta((\|\bfA^*\|_\infty^2+\epsilon^{10}) K^3p^2\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^2(\|\bfA^*\|_\infty+1)^2\epsilon^{-2})$, with high probability SGD after $T$ iterations returns 
$$\mathbb{E}_{(\bfe_g,\bfX,y)\sim\mathcal{D}}[L( F(\bfe_g, \bfX,\bfW^{out}),y)]\leq OPT+\epsilon$$

\fi


 



\begin{theorem}(Generalization of training three-layer GCNs with sampling)\label{thm:three_sampling}
 
If Assumption \ref{ap_sampling} is met, and all other conditions in Theorem \ref{thm:three} are met, then
\begin{equation}
{E}_{(\bfe_g,\bfX,y)\in\mathcal{D}}L(\lambda_T F(\bfe_g,\bfX;\bfW_T^{(out)}, \bfV_T^{(out)}),y)\leq (1+\gamma) \mathrm{OPT}+\epsilon_0
    \end{equation}
     
\end{theorem}
where $\bfW_T^{(out)}$, $\bfV_T^{(out)}$ are the returned weight matrices. 
% for every constant $\gamma\in(0,\frac{1}{4}]$, every $\epsilon_0\in(0,\frac{1}{100}]$, every $\epsilon\in(0,\frac{1}{Kp_1p_2^2\mathcal{C}_s(\Phi, p_2\mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty))\mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty)(\|\bfA^*\|_\infty+1)})$, there exist 
\iffalse
\begin{equation}
\begin{aligned}
M=\text{poly}(&\mathcal{C}_s(\Phi, p_2\mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty)), \mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty), \\
&\|\bfA^*\|_\infty, 1/\epsilon) 
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
  \textrm{and }  
    N_0= &\epsilon^{-2}\|\bfA^*\|_\infty^4(1+p\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)\sqrt{\|\bfA^*\|_\infty^2+1})^4\\
    &K^2(1+\delta)^4\log N
\end{aligned}
\end{equation}

such that  as long as $m_1=m_2=m\geq M$, and $n_0 \geq N_0$, % as long as
%$$N_0= \epsilon^{-2}(1+\|\bfA\|_\infty)^4 K^2(1+\delta^2)^2\log N$$
there is a choice $\eta=1/\text{poly}(\|\bfA^*\|_\infty, K, m)$ and $T=\text{poly}(\|\bfA^*\|_\infty, K, m)$ such that with probability $\geq 99/100$,
$$\mathbb{E}_{(\bfe_g,\bfX,y)\in\mathcal{D}}L(\lambda_T F(\bfe_g,\bfX;\bfW_T^{(out)}, \bfV_T^{(out)}),y)\leq (1+\gamma)OPT+\epsilon_0$$




Note that from Assumption \ref{ap_sampling}, the total number of sampled nodes can be much less $N$, as long as $p_l$'s are small, % while the generalization performance is maintained, 
indicating the success of sampling. 
To understand the sampling requirement in (\ref{eqn:ll}) better, consider a special case that %$\bfA^*=\bfA$, which means 
$p^*_l=1$, and $N_l$ is order $N$   for all $l$. Then % for a larger $l$,  $\Phi_l$ is larger , then 
$l_l$ is larger with a larger $d_l$. That means the higher-degree groups are sampled more often than lower-degree groups in this case.  This shares the same intuition as FastGCN \citep{CMX18}, which also samples high-degree nodes with a higher probability. 
\fi
%Specifically, although the nodes in group $L$ should be almost all sampled, the nodes in other groups $l$ ($l<L$) can be very small as long as $p^*_l$ is small enough. Therefore, our sampling strategy focuses on the high-degree group and samples less from low-degree groups. Although different in the actual strategy, our sampling method  shares the same intuition as FastGCN \cite{}, which also samples high-degree nodes with a higher probability. 


Theorems  \ref{thm:two_sampling} and \ref{thm:three_sampling} indicate that even when the sampled nodes is much less than $N$, it is still possible to learn a GCN with a small generalization error. The intuition is that  the actual correlations among nodes is not as intense as the adjacency matrix $\bfA$ and can be properly incorporated in training even with graph sampling. 



%provide a theoretical explanation about the empirical observations that graph sampling does not degrade the generalization performance in some datasets. That may be because in these datasets,    the sampling method is consistent with the   $\bfA^*$ in target function. 

%Because the ground truth A* in the target function is not nessearyli A, training usuing A do not always provide the best erpformance despite the high computational cost. Threom shows that if the probabily of samping stateg is consistent with A*, one can have guarntted genearliztaion performance even if only a small portion of nodes each iteration. 
%
%assumes the sampling probabaly P* exactly, and such requirement can be relaxed minorly 

==> three_layer.tex <==
\section{Training three-layer GCNs without sampling}\label{sec:three}

\PY{Any reason we first mention 2-layer then 3-layer? I think we can directly state the result of 3-layer. 2-layer is a special case and can be put in the appendix}

Now we consider training three-layer GCNs.
\textbf{Concept class and target function $F^*$}. 
Consider target functions $F^*: \mathbb{R}^N\times  \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^K$:
\begin{equation}\label{eqn:concept2}
\begin{aligned}
&F^*=(f_1^*,f_2^*,\cdots, f_K^*), \\
&f_r^*(\bfe_g, \bfX)=\bfe_g^\top \sum_{k\in[p_1]}c_{k,r}^*\Phi\Big(\bfA^*\sum_{j\in[p_2]}v_{1,k,j}^*\phi_{1,j}(\bfA^*\bfX\bfw_{1,j}^*)\Big)\\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \odot \Big(\bfA^*\sum_{l\in[p_2]}v_{2,k,l}^*\phi_{2,l}(\bfA^*\bfX\bfw_{2,l}^*)\Big),\ 
\forall r\in[K],
\end{aligned}
\end{equation}
where each $\phi_{1,j}$, $\phi_{2,j}$, $\Phi_i$: $\mathbb{R}\rightarrow\mathbb{R}$ is infinite-order smooth. The concept class contains all functions  $F^*$ in the form of   (\ref{eqn:concept2}) with any parameters 
$\bfw_{1,j}^*, \bfw_{2,j}^*\in\mathbb{R}^d$,  $\bfv_{1,k}^*, \bfv_{2,k}\in\mathbb{R}^{p_2}$,  $c_{k,r}^*\in\mathbb{R}$, $\forall j \in [p_2]$, $\forall k \in [p_1]$, and $\forall r \in [K]$, that satisfy $\|\bfw_{1,j}^*\|=\|\bfw_{2,j}^*\|=\|\bfv_{1,k}^*\|=\|\bfv_{2,k}^*\|=1$ and $|c_{k,r}^*|\leq1$. Let 
$
\mathrm{OPT}= \mathbb{E}\limit_{(e_g, \bfX, y)\sim \mathcal{D}} L (F^*(e_g, \bfX), y)$ 
be the smallest population risk achieved by the best target function in the concept class.
The standard three-layer GNNs with 
\begin{equation}
 f_r^*(\bfe_g, \bfX)=\bfe_g^\top \sum_{k\in[p_1]}c_{k,r}^*\Phi(\bfA^*\sum_{j\in[p_2]}v_{1,k,j}^*\phi_{1,j}(\bfA^*\bfX\bfw_{1,j}^*)), \forall r \in [K]
\end{equation}
are only special cases of (\ref{eqn:concept2}). 
 
\iffalse
 \begin{equation}\label{eqn:concept2}
F^*=(f_1^*,f_2^*,\cdots, f_K^*), \\
f_r^*(\bfe_g, \bfX)= \sum_{k\in[p_1]}c_{k,r}^*\Phi(\bfa_g^\top\sum_{j\in[p_2]}v_{1,j}^*\phi_{1,j}(\bfA^*\bfX\bfw_{1,j}^*))\bfa_g^\top\sum_{l\in[p_2]}v_{2,l}^*\phi_{2,l}(\bfA^*\bfX\bfw_{2,l}^*) 
\forall l\in[K],
\end{equation}
where each $\phi_{1,j}$, $\phi_{2,j}$, $\Phi_i$: $\mathbb{R}\rightarrow\mathbb{R}$ is infinite-order smooth. The concept class contains all functions  $F^*$ in the form of   (\ref{eqn:concept2}) with any parameters 
$\bfw_{1,j}^*, \bfw_{2,j}^*\in\mathbb{R}^d$, $\bfv_{1,j}^*, \bfv_{2,j}\in\mathbb{R}^{p_2}$, $c_{k,r}^*\in\mathbb{R}$ that satisfy $\|\bfw_{1,j}^*\|=\|\bfw_{2,j}^*\|=\|\bfv_{1,j}^*\|=\|\bfv_{2,j}^*\|=1$ and $|c_{k,r}^*|\leq1$. Let 
$
\mathrm{OPT}= \mathbb{E}\limit_{(e_g, \bfX, y)\sim \mathcal{D}} L (F^*(e_g, \bfX), y)$ 
be the smallest population risk achieved by the best target function in the concept class.  %OPT reflects the average risk of estimating the unknown labels using the best target function. OPT decreases when the complexity of the concept class increases. 
\fi


 
 \textbf{Learner network} We train a three-layer network $F: \mathbb{R}^N\times   \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^K$ with
\begin{equation}\label{eqn:twolayer}
\begin{aligned}
&F=(f_1,f_2,\cdots,f_K),\\
&f_r(\bfe_g,\bfX)=\bfe_g^\top \sigma(  \bfr+\bfB_2)\bfc_r, \quad \forall r \in [K], 
\end{aligned}
\end{equation}
\begin{equation}
\bfr= \bfA\sigma(\bfA\bfX\bfW+\bfB_1)\bfV 
\end{equation}
%for $r\in[K]$, 
where % $\sigma(x)=\max(x,0)$ is the ReLU activation, 
$\bfW\in\mathbb{R}^{d\times m_1}$ and $\bfV\in\mathbb{R}^{m_1\times m_2}$ represent the weights of $m_1$ and $m_2$ hidden nodes in each layer, respectively.   $\bfB_1\in\mathbb{R}^{N\times m_1}$  and  $\bfB_2\in\mathbb{R}^{m_1\times m_2}$ represent the bias matrices.  $\bfc_r\in\mathbb{R}^m$ is the output weight vector. % In the training process, we only update $\bfW$ and $\bfV$, while keeping others as initial values.  %Thus, 
We write $F$ and $f_r$ as $F(e_g,\bfX; \bfW, \bfV)$ and $f_r(e_g,\bfX ;\bfW,\bfV)$, as we only update $\bfW$ and $\bfV$ in training, while keeping others as initial values.. Given training data $\mathcal{Z}=\{z^1,..., z^{n_0}\}$, the objective is to find $\bfW$ and $\bfV$ such that the population risk of the learner network, denoted by $\mathbb{E}_{(e_g, \bfX, y)\sim \mathcal{D}} L (F(e_g, \bfX;\bfW,\bfV), y)$, is at most $\mathrm{OPT}+\epsilon$.
 

\iffalse

\textbf{Learner network} We train a three-layer network $F: \mathbb{R}^N\times   \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^K$ with
\begin{equation}\label{eqn:threelayer}
F=(f_1,f_2,\cdots,f_K),\ \ \ \ f_r(\bfe_g,\bfX)=\bfe_g^\top \sigma(r+\bfB_2)\bfc_r \quad \forall r \in [K], 
\end{equation}
\begin{equation}
\bfr=\bfA\sigma(\bfA\bfX_i\bfW+\bfB_1)\bfV 
\end{equation}
%for $r\in[K]$, 
where %$\sigma(x)=\max(x,0)$ is the ReLU activation,
$\bfW\in\mathbb{R}^{d\times m}$ represents the weights of the $m$ hidden nodes in two layers, respectively.   $\bfB\in\mathbb{R}^{N\times m}$ is the bias matrix, and $\bfc_r\in\mathbb{R}^m$ is the output weight vector. In the training process, we only update $\bfW$, and keep the values of $\bfB\in\mathbb{R}^{N\times m}$ and $\bfc_r\in\mathbb{R}^m$ as initial values.  Thus, we write $F$ and $f_r$ as $F(e_g,\bfX ;\bfW)$ and $f_r(e_g,\bfX ;\bfW)$. Given training data $\mathcal{Z}=\{z^1,..., z^{n_0}\}$, the objective is to find $\bfW$ such that the population risk of the learner network, denoted by $\mathbb{E}\limits_{(e_g, \bfX, y)\sim \mathcal{D}} L (F(e_g, \bfX;\bfW), y)$, is at most $\mathrm{OPT}+\epsilon$.

\noindent \textbf{Learner network} We train a network $F: \mathbb{R}^N\times \mathbb{R}^{N\times N}\times \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^K$ with
$$F(\bfe_g, \bfA,\bfX_i, \bfW,\bfB)=\bfe_g^\top \sigma(\bfr+\bfB_2)\bfC$$
$$\bfr=\bfA\sigma(\bfA\bfX_i\bfW+\bfB_1)\bfV$$
where $\bfW\in\mathbb{R}^{d\times m_1}$, $\bfB=(\bfB_1,\bfB_2)$, $\bfB_1\in\mathbb{R}^{N\times m_1}$, $\bfV\in\mathbb{R}^{m_1\times m_2}$, $\bfB_2\in\mathbb{R}^{N\times m_2}$, $\bfC\in\mathbb{R}^{m_2\times K}$. Entries of $\bfW^{(0)}$ are i.i.d.   Gaussian  from $\mathcal{N}(0,\frac{1}{m_1})$, and entries of $\bfV^{(0)}$ are i.i.d.  Gaussian  from $\mathcal{N}(0,\frac{1}{m_2})$. We generate $\bfB_1^{(0)}$ (or $\bfB_2^{(0)}$) by initializing one row vector from $\mathcal{N}(0,\frac{1}{m_1}\bfI)$ (or $\mathcal{N}(0, \frac{1}{m_2}\bfI)$) and other rows equal to this row. Entries of $\bfC$ are i.i.d. random Gaussians from $\mathcal{N}(0, \epsilon_c^2)$ for some fixed $\epsilon_c\in(0,1]$. 
\fi

\textbf{Technical challenges of three-layer GCNs}
The main difficulty in analyzing three-layer GCNs is that due to the nonlinear iteration of $\bfW$ and $\bfV$, the risk function is nonconvex. The convexity plays a critial role in many exiting analyses of GCNs. For instance, in the two-layer case in Section \ref{sec:two}, if the SGD iterates stay close enough to the initialization, the risk function is convex in $\bfW$, and thus the iterates converge to the global minimum. The analyses in \cite{ZWLC20} requires a special initialization in the local convex region of the global minimum. The NTK approach in \cite{DHPSWX19} considers the limiting case that the interactions across layers are negligible. Here, we directly address the non-convexity of the risk function in $\bfW$ and $\bfV$. The main idea is to add weight decay and regularization such that with a proper regularization, any second-order critical point is almost a global minimum.

%NTK, and other convexity. No longer convex due to interactacions of weights W and V. Introduce weight decay to get out of local minimum and regularization for what? 

\textbf{Learning Algorithm}
 Entries of $\bfW^{(0)}$ are i.i.d.    from $\mathcal{N}(0,\frac{1}{m_1})$, and entries of $\bfV^{(0)}$ are i.i.d.     from $\mathcal{N}(0,\frac{1}{m_2})$. 
 $\bfB_1^{(0)}$ (or $\bfB_2^{(0)}$) is initialized to be an all one vector multiplying a row vector with i.i.d. samples from    $\mathcal{N}(0,\frac{1}{m})$  (or $\mathcal{N}(0, \frac{1}{m_2})$). Entries of $c_r$ are  drawn i.i.d.   from $\mathcal{N}(0, \epsilon_c^2)$ for some fixed $\epsilon_c\in(0,1]$. 
 
 %We only update $\bfW$ and $\bfV$ using SGD with weight decay and regularization. To facilitate the theoretical analyses, we also include Gaussian smoothing and Dropout. Specifically,
 
 
 In each round $t=1, ..., T$, we use noisy SGD with step size $\eta$ for $T_w$ iterations to minimize the objective function $\hat{L}$ with some fixed $\lambda_{t-1}$, where $\lambda_0=1$, and the weight decays with $\lambda_{t}=\eta\lambda_{t-1}$.
\begin{equation}\label{eqn:hatL}
\begin{aligned}
    &\hat{L}(\lambda_{t-1};\bfW,\bfV)\\
    =&L(\lambda_{t-1}F(\bfe_g, \bfX;\bfW^{(0)}+\bfW^\rho+\bfW\boldsymbol{\Sigma}, \bfV^{(0)}+\bfV^\rho+\boldsymbol{\Sigma}\bfV))\\
    &+R(\sqrt{\lambda_{t-1}}\bfW,\sqrt{\lambda_{t-1}}\bfV)
\end{aligned}
\end{equation}
 
 
 
 Note that $\lambda F$  in (\ref{eqn:hatL}) is equivalent to replacing $\bfW$ and $\bfV$ with   $\sqrt{\lambda} \bfW$ and $\sqrt{\lambda} \bfV$, because ReLU network is homogeneous.  $\bfW^{\rho}$ and $\bfV^{\rho}$ are small perturbation matrices with entries i.i.d. drawn from $\mathcal{N}(0, \sigma_w^2)$ and $\mathcal{N}(0, \sigma_v^2)$, respectively. Noisy SGD is vanilla SGD plus Gaussian perturbation. Both are common tricks in the  literature
of theoretical analyses of non-convex optimization, see, e.g. \citep{GHJY15},  and are not needed in practice.  
  $\sigma \in \mathbb{R}^{m_1\times m_1}$ is   a random diagonal matrix with diagonal entries uniformly drawn from $\{1, -1\}$. This is similar to the practical Dropout \citep{} technique that randomly masks out neurons and is also introduced for the theoretical analysis only.
 $\hat{L}$ includes an additional regularization, defined as %is the regularizer with. 
  \begin{equation}
    R(\sqrt{\lambda}\bfW,\sqrt{\lambda}\bfV)=\lambda_w\|\sqrt{\lambda}\bfW\|_{2,4}^4+\lambda_v\|\sqrt{\lambda}\bfV\|_F^2
\end{equation}
for some positive $\lambda_w$ and $\lambda_v$. 
As shown in \citep{ALL19}, $\|\cdot\|_{2,4}$ is used for the analysis to drive the weights to be evenly distributed among neurons. The practical regularization $\|\cdot\|_F$ has the same effect in empirical results, while the theoretical justification is open.  Let $\bfW^{out}$ and $\bfV^{out}$ denote the returned weights by Algorithm xx after round $T$. then the generalization performance of the returned model is shown in the following theorem. 
 
 
 
\begin{theorem}(Generalization of training three-layer GCNs)
\label{thm: node_3}
The parameters are selected as in Table xxx. 
For every constant $\gamma\in(0,\frac{1}{4}]$, every $\epsilon_0\in(0,\frac{1}{100}]$, every $\epsilon\in(0,\frac{1}{Kp_1p_2^2\mathcal{C}_s(\Phi, p_2\mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty))\mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty)(\|\bfA^*\|_\infty+1)})$, there exist 
\begin{equation}
\begin{aligned}
M=\text{poly}(&\mathcal{C}_s(\Phi, p_2\mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty)), \mathcal{C}_s(\phi,1+\|\bfA^*\|_\infty), \\
&\|\bfA^*\|_\infty, 1/\epsilon)
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
  \textrm{and }   
    N_0=& \epsilon^{-2}\|\bfA^*\|_\infty^4(1+p\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)\sqrt{\|\bfA^*\|_\infty^2+1})^4\\
    \cdot K^2(1+\delta)^4\log N
\end{aligned}
\end{equation}
such that  as long as $m_1=m_2=m\geq M$, and $n_0 \geq N_0$, % as long as
%$$N_0= \epsilon^{-2}(1+\|\bfA\|_\infty)^4 K^2(1+\delta^2)^2\log N$$
there is a choice $\eta=1/\text{poly}(\|\bfA^*\|_\infty, K, m)$ and $T=\text{poly}(\|\bfA^*\|_\infty, K, m)$ such that with probability $\geq 99/100$,
 \begin{equation}
     \mathbb{E}_{(\bfe_g,\bfX,y)\in\mathcal{D}}L(\lambda_T F(\bfe_g,\bfX;\bfW_T^{(out)}, \bfV_T^{(out)}),y)\leq (1+\gamma)\mathrm{OPT}+\epsilon_0 
 \end{equation}
\end{theorem}

Theorem shows that with the weights $\sqrt{\lambda_T}\bfW_T^{(out)}$ and $\sqrt{\lambda_T}\bfV_T^{(out)}$, a three-layer GCN achieves a population risk of $\mathrm{OPT}+\epsilon_0$ for any small enough  $\epsilon_0$. This is a stronger result than the average generalization result for two-layer GCNs in  (\ref{eqn:twolayer}). Moreover, 
  three-layer GCNs can  approximate a much richer class of target functions in (\ref{eqn:concept2}) than those for two-layer GCNs in (\ref{eqn:concept}). Similar to the two-layer GCNs, the sample complexity for three-layer GCNs is   polynomial in $\|\bfA^*\|$ and $\delta$. To the best of our knowledge, this is the first sample complexity and generalization analysis for three-layer GCNs.
  
  
  %Second, () shows that the returne
 %
% We generate $\bfB_1^{(0)}$ (or $\bfB_2^{(0)}$) by initializing one row vector from $\mathcal{N}(0,\frac{1}{m_1}\bfI)$ (or $\mathcal{N}(0, \frac{1}{m_2}\bfI)$) and other rows equal to this row. Entries of $\bfC$ are i.i.d. random Gaussians from $\mathcal{N}(0, \epsilon_c^2)$ for some fixed $\epsilon_c\in(0,1]$. 

==> two_layer.tex <==
\section{Training two-layer GCNs without sampling}\label{sec:two}

%We first state the following general target function, and the one-hidden-layer neural network can be considered as a special case. 
We first discuss training two-layer GCNs as a warmup for the more complicated three-layer case. Here we  use vanilla SGD to minimize the empirical risk directly, and our result  two-layer GCNs is of independent interest itself. % as it considers a more general and practical setup and then existing results on two-layer GCNs such as Du. et. al 2019 and Zhang et al 2019. 


\textbf{Concept class and target function $F^*$} %(\bfe_g, \bfX)$}. 
Consider target functions $F^*: \mathbb{R}^N\times  \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^K$:
\begin{equation}\label{eqn:concept}
\begin{aligned}
&F^*=(f_1^*,f_2^*,\cdots, f_K^*),\\
&f_r^*(\bfe_g, \bfX)=\bfe_g^\top\sum_{i=1}^p c_{i,r}^*(\phi_i(\bfA^*\bfX\bfw_{1,i}^*)\\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \odot (\bfA^*\bfX\bfw_{2,i}^*)), \quad \forall r \in [K], 
\end{aligned}
\end{equation}
%for $r\in[K]$,  %where $\bfe_g=(0,\cdots,0,1,0,\cdots,0)$ with its $g$-th entry equal to 1 $(g=1,...,N)$, 
where each $\phi_i: \mathbb{R} \rightarrow \mathbb{R}$ is infinite-order smooth, and $\bfA^*$ is a fixed matrix. %with \tcr{please add the constraint on the norm of A}. 
The concept class contains all functions  $F^*$ in the form of   (\ref{eqn:concept}) with any parameters $\bfw_{i}^*$ and $c_{i,r}^*$.  % \tcr{why do we need this? We assume $\|\bfw_{1,i}^*\|=\|\bfw_{2,i}^*\|=1$ and $|c_{i,r}^*|\leq 1$ for simplicity.} 
Let 
\begin{equation}
\mathrm{OPT}= \mathbb{E}\limit_{(e_g, \bfX, y)\sim \mathcal{D}} L (F^*(e_g, \bfX), y)
\end{equation}
be the \textit{smallest} population risk achieved by the best target function in the concept class.  OPT reflects the average risk of estimating the unknown labels using the best target function. %OPT decreases when the complexity of the concept class increases. 
  The standard two-layer GCNs with 
\begin{equation}
 f_r^*(\bfe_g, \bfX)=\bfe_g^\top\sum_{i=1}^p c_{i,r}^*(\phi_i(\bfA^*\bfX\bfw_{1,i}^*), \forall r \in [K]
\end{equation}
are only special cases of (\ref{eqn:concept}). 
 

  

%$g$ is randomly picked from $\{1,\cdots,N\}$. Here $\bfX_i$ is the $i$-th realization in the training set. We assume that there exists a sparse subgraph $\bfA^*$ of $\bfA$ that can express the full $\bfA$ during training. The set of vertices of $\bfA^*$ is denoted as $\bfs^*$. Different weights are assigned to the vertices in $\bfs^*$ as $\{q_j^*\}_{j=1}^N$ with $\sum_{u_j\in\bfs^*}q_j^*=1$ and $\sum_{u_j\notin\bfs^*}q_j^*=0$. 
 
 
\textbf{Learner network} We train a two-layer network $F: \mathbb{R}^N\times   \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^K$ with
\begin{equation}\label{eqn:twolayer}
\begin{aligned}
&F=(f_1,f_2,\cdots,f_K),\\
&f_r(\bfe_g,\bfX)=\bfe_g^\top \sigma(\bfA \bfX \bfW+\bfB)\bfc_r \quad \forall r \in [K], 
\end{aligned}
\end{equation}
%for $r\in[K]$, 
where $\sigma(x)=\max(x,0)$ is the ReLU activation, $\bfW\in\mathbb{R}^{d\times m}$ represents the weights of the $m$ hidden nodes,  $\bfB\in\mathbb{R}^{N\times m}$ is the bias matrix, and $\bfc_r\in\mathbb{R}^m$ is the output weight vector. In the training process, we only update $\bfW$, and keep the values of $\bfB\in\mathbb{R}^{N\times m}$ and $\bfc_r\in\mathbb{R}^m$ as initial values.  Thus, we write $F$ and $f_r$ as $F(e_g,\bfX ;\bfW)$ and $f_r(e_g,\bfX ;\bfW)$. Given training data $\mathcal{Z}=\{z^1,..., z^{n_0}\}$, the objective is to find $\bfW$ such that the population risk of the learner network, denoted by $\mathbb{E}\limits_{(e_g, \bfX, y)\sim \mathcal{D}} L (F(e_g, \bfX;\bfW), y)$, is at most $\mathrm{OPT}+\epsilon$.  


We remark that $\bfA^*$ in the concept class (\ref{eqn:concept}) and $\bfA$ in the learner network (\ref{eqn:twolayer}) are not necessarily the same.   $\bfA$ is   the (symmetric) normalized adjacency matrix of the un-directed graph $\mathcal{G}$.  $\bfA^*$ reflects the target correlations in neighboring nodes and can be asymmetric. %In a general setting, 
$\bfA^{*\top}$ can be viewed as an adjacency matrix of a weighted directed graph $\mathcal{G'}$, where each un-directed edge in $\mathcal{G}$ corresponds to two directed edges in $\mathcal{G}$ with possibly different weights. We consider the case that $\bfA=\bfA^*$ in Sections \ref{sec:two} and \ref{sec:three} and defer the discussion of  $\bfA=\bfA^*$ in Section \ref{sec: sampling}. 

\textbf{Learning Algorithm}

%add initialization of W and B and cr, and sgd step. Add an Algorithm block, which most likely will appear in appendix. 
We initialize $\bfW^{(0)}$ with i.i.d. entries  from Gaussian   $\mathcal{N}(0,\frac{1}{m})$. $\bfB^{(0)}$ is initialized to be an all one vector multiplying a row vector with i.i.d. samples from    $\mathcal{N}(0,\frac{1}{m})$. Thus, all rows of  $\bfB^{(0)}$ are the same. %and other rows equal to this row. 
Entries of $c_r$ are  drawn i.i.d.   from $\mathcal{N}(0, \epsilon_c^2)$ for some fixed $\epsilon_c\in(0,1]$. 
A batch SGD with batch size 1 is employed to update $\bfW$ with step size $\eta$ for $T$ iterations. Let $\bfW^t$ denote the returned weight matrix after iteration $t$.

Theorem \ref{thm:two} summarizes our result for the generalization performance of   two-layer GCNs learned by SGD. With enough neurons and node labels, % are both larger than the corresponding thresholds, which are both polynomials of $\|\bfA^*\|_\infty$, then 
SGD with a proper step size and enough  iterations returns a model with a population risk that is at most $OPT+\epsilon$. 


\begin{theorem}[Generalization of training two-layer GCNs without sampling]\label{thm:two} 
%\begin{theorem}\label{thm: node_2_layer}
For every $\epsilon\in(0,K^{-\frac{13}{2}}p^{-4}\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^{-4}(\|\bfA^*\|_\infty+1)^{-4}\|\bfA^*\|_\infty^{-1})$, there exists
\begin{equation}
M_0=\Theta\big(\epsilon^{-6}K^{12}p^{8}\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^{8}(\|\bfA^*\|_\infty+1)^{8}\|\bfA^*\|_\infty^4\big)
\end{equation}
\begin{equation}
N_0= \epsilon^{-2} K^7 p^4\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^4(\|\bfA^*\|_\infty^2+1)^2\|\bfA^*\|_\infty^4(1+\delta^2)\log N
\end{equation}
such that  as long as $m\geq M_0$ and $n_0\geq N_0$, choosing $\epsilon_c=\Theta(1)$, $\eta=\Theta(\frac{\epsilon}{m\epsilon_c^2 K\|\bfA\|_\infty^2})$ and $T=\Theta(\|\bfA^*\|_\infty^2 K^3p^2\mathcal{C}_s(\phi,\|\bfA^*\|_\infty)^2(\|\bfA^*\|_\infty+1)^2\epsilon^{-2})$, with high probability SGD after $T$ iterations returns 
\begin{equation}\label{eqn:twolayer}
\mathbb{E}[\frac{1}{T}\sum_{t=1}^{T}\mathbb{E}_{(\bfe_g,\bfX,y)\sim\mathcal{D}}L( F(\bfe_g, \bfX, \bfW^t),y)]\leq    \mathrm{OPT}+\epsilon 
\end{equation}
\end{theorem}
where the first expectation in (\ref{eqn:twolayer}) is taken over the randomness of SGD.   (\ref{eqn:twolayer}) shows that the average population risk of the returned models in  all iterations is less than  $\mathrm{OPT}+\epsilon$, then the population risk of at least one model less than  $\mathrm{OPT}+\epsilon$. In the three-layer case in Section \ref{sec:three}, we will quantify the population risk of the finally returned model directly, but the proof will be more involved.

Theorem \ref{thm:two} shows that the required sample complexity is  polynomial in $\|\bfA^*\|$ and $\delta$, where $\delta$ is the maximum node degree. Then as long as  $\|\bfA^*\|$ and $\delta$ are   $O(N^\alpha)$ for some small $\alpha$ in $(0,1)$, say $\alpha=1/10$,  then 
one can accurately infer the unknown labels   from a small percentage of labeled nodes. In general, the sample complexity increases when the node degree increases, coinciding with the intuition that a stronger correlation among nodes is more challenging to learn.    Moreover, the sample complexity is weakly dependent of the required number of neurons $M$, in the order of ploy($\log m$). 


The dependence of the sample complexity on the graph structures is also analyzed in \citep{ZWLC20}. However, \citep{ZWLC20} requires a special initialization via the tensor method while our analysis applies to the vanilla SGD. Moreover, the sample complexity bound in \citep{ZWLC20} is a polynomial of $m$, which does not apply to the practical case of  over-parameterization.   Lastly, Theorem \ref{thm:two} applies to learning a general class of target functions in (\ref{eqn:concept}) with two-layer neural networks as a special case, while \citep{ZWLC20} focuses on two-layer GCNs only. 

\PY{Al go 1: better replace training data with labeled nodes; graph should be an input; 'sampling SGD' is a weird wording. Better use SGD with node sampling.}

\begin{algorithm}

\caption{Sampling SGD for two-layer networks}

\begin{algorithmic}[1]\label{gd}
\STATE{\textbf{Input: }} 
 Training data $\mathcal{Z}$, initialization $\bfW^{(0)}$, $\bfB^{(0)}$, step size $\eta$.
\STATE $\bfW_0=0$
\FOR{$t=0,1,\cdots,T-1$}
\STATE Randomly sample $\bfz=(\bfX_i, \bfy_i)$ from $\mathcal{Z}$ and generate $\bfA_t$.
%\vspace{-0.1in}
%\textcolor{red}{$$\bfW_{t+1}=\bfW_t-\eta_0\widetilde{\nabla f_n(\bfW_t)}=\bfW_t-\eta_0\Big(\nabla f_n(\bfW^*)+\frac{1}{n}\sum_{i=1}^n \nu_i\Big)$$}
\begin{equation}\label{eqn:gradient}
\begin{aligned}
\bfW_{t}&=\bfW_{t-1}-\eta\frac{\partial}{\partial \bfW}L(F(\bfA_t, \bfX_i,\bfW^{(0)}+\bfW_{t-1}), \bfy_i)
\end{aligned}
\end{equation}
\ENDFOR
%\vspace{-0.1in}
\STATE{\textbf{Output: }} $\bfW^{out}=\bfW^{(0)}+\bfW_T$
\end{algorithmic}
\end{algorithm}

%\subsection{Theoretical result and insights}
